Non-Photorealistic Rendering of Layered Materials: A Multispectral Approach

We present multispectral rendering techniques for visualizing layered materials found in biological specimens. We are the first to use acquired data from the near-infrared and ultraviolet spectra for non-photorealistic rendering (NPR). Several plant and animal species are more comprehensively understood by multispectral analysis. However, traditional NPR techniques ignore unique information outside the visible spectrum. We introduce algorithms and principles for processing wavelength dependent surface normals and reflectance. Our registration and feature detection methods are used to formulate stylization effects not considered by current NPR methods including: Spectral Band Shading which isolates and emphasizes shape features at specific wavelengths at multiple scales. Experts in our user study demonstrate the effectiveness of our system for applications in the biological sciences.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> expert.tex <==
\section{Applications}
\label{sec:applications}

The whale cranium in Figures~\ref{fig:teaser} and~\ref{fig:contrastlightdata} is uniquely suited for demonstrating applications of our algorithms because it encodes biological traits and artistic features. The normal maps capture sutures, used determine age. Cracks and pores from exposure to elements are clues about provenance. Figure~\ref{fig:sailboat} illustrates multiscale, multispectral curvature shading and line extraction for analyzing the story engraved artwork (\emph{scrimshaw}). Curvature shading emphasizes shapes (grooves and hill features). Combined with spectral band shading, extracted curvatures can reveal markings that are not detectible under visible light due to the white monochrome color, weathering, and erosion. Examination of \emph{organic walled fossils} which are composed of outer layers of carbon-based proteinaceous material is another application that requires isolation of spectral wavelengths.  In this case, external layers are easily penetrable by near-infrared waves.  


\input{../fig-sailboat}



Our algorithms are generalizable to disciplines like forensics where visualizing bitemarks, injury patterns , shoeprints and latent fingerprints are important. 


Dynamic near-infrared enhancement lights can be used to study specific internal structures by emphasizing NIR features while deemphasizing visible features (Figure~\ref{fig:shadinglights} a). Dynamic spectral band shading may be used to visualize fossil features under the sediment layers while dynamic focused lights are useful for isolating specific features (Figure~\ref{fig:shadinglights} c). Figure~\ref{fig:sbsbandcontrol} demonstrates spectral band shading controls for isolating different wavelengths. Natural history artifacts may exhibit naturally occurring pigments that depict customs or communicate information. These pigments often behave differently under different electromagnetic wavelengths. Figure~\ref{fig:sbsspectralcontrol} is an application of spectral band shading for analyzing subsurface detail below these pigments. Note that the red dye is not visible in the near-infrared image (Figure~\ref{fig:realexample} \emph{right}). Figure~\ref{fig:shadingmodelscompare} compares spectral band shading to classic NPR shading techniques. Figure~\ref{fig:irblending} shows the flexibility of the pipeline and demonstrates near-infrared blending to enhance the circle patterns on the underside of the butterfly wing. The painting effect was created by applying joint bilateral filtering to  visible color and normals and light filtering to near-infrared \hbox{2-D} spectral data. Lambertian shading was computed with visible color and normals using a light direction that illuminated the entire specimen. A per pixel, per channel blending multiplies a blending color parameter with the quantized original near-infrared \hbox{2-D} spectral data (to preserves details lost in smoothing). Quantization using k-means clustering gives the toon-like effect. 












 



==> fig-bispectralnormals.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.9\hsize]{./images/micro/bispectralnormals-v003.eps}
\setlength{\belowcaptionskip}{-10pt} 
\caption{\label{fig:bispectralnormals}%
(left to right) normals: visible and combined bispectral, reflectance: visible and bispectral}
\end{figure}





